Easing Embedding Learning by Comprehensive Transcription of Heterogeneous Information Networks

Heterogeneous information networks (HINs) are ubiquitous in real-world applications. In the meantime, network embedding has emerged as a convenient tool to mine and learn from networked data. As a result, it is of interest to develop HIN embedding methods. However, the heterogeneity in HINs introduces not only rich information but also potentially incompatible semantics, which poses special challenges to embedding learning in HINs. With the intention to preserve the rich yet potentially incompatible information in HIN embedding, we propose to study the problem of comprehensive transcription of heterogeneous information networks. The comprehensive transcription of HINs also provides an easy-to-use approach to unleash the power of HINs, since it requires no additional supervision, expertise, or feature engineering. To cope with the challenges in the comprehensive transcription of HINs, we propose the HEER algorithm, which embeds HINs via edge representations that are further coupled with properly-learned heterogeneous metrics. To corroborate the efficacy of HEER, we conducted experiments on two large-scale real-words datasets with an edge reconstruction task and multiple case studies. Experiment results demonstrate the effectiveness of the proposed HEER model and the utility of edge representations and heterogeneous metrics. The code and data are available at https://github.com/GentleZhu/HEER.

==> Makefile <==
TARGET = edge_rep

pdf:
	pdflatex $(TARGET) && bibtex $(TARGET) && pdflatex $(TARGET) && \
	pdflatex $(TARGET)
	open $(TARGET).pdf
clean:
	rm -f *.aux *.log *.blg *.bbl *~ *.dvi *.out *.nav *.snm *.toc *.brf *.backup $(TARGETS)


==> discussion.tex <==
%!TEX root = mvn2vec.tex

\section{Discussion}
\cmg{May drop the section.} In the applications that have using HIN have showed benefit over homogeneous networks are those with accurate and distinctive type information. Accurate as in bibliographic networks or social networks where types are self-explanatory in nature, in stead of examples like types inferred from text where are unlikely to be completely accurate. Distinctive as these types describe different natures of the node such as person against location, instead of protein against gene.

When the type is inaccurate or not distinctive, using homogeneous network embedding algorithms may generate results as good.

